PhantomLiDAR: Cross-modality Signal Injection Attacks against LiDAR

LiDAR (Light Detection and Ranging) is a pivotal sensor for autonomous driving, offering precise 3D spatial information. Previous signal attacks against LiDAR systems mainly exploit laser signals. In this paper, we investigate the possibility of cross-modality signal injection attacks, i.e., injecting intentional electromagnetic interference (IEMI) to manipulate LiDAR output. Our insight is that the internal modules of a LiDAR, i.e., the laser receiving circuit, the monitoring sensors, and the beam-steering modules, even with strict electromagnetic compatibility (EMC) testing, can still couple with the IEMI attack signals and result in the malfunction of LiDAR systems. Based on the above attack surfaces, we propose the PhantomLiDAR attack, which manipulates LiDAR output in terms of Points Interference, Points Injection, Points Removal, and even LiDAR Power-Off. We evaluate and demonstrate the effectiveness of PhantomLiDAR with both simulated and real-world experiments on five COTS LiDAR systems. We also conduct feasibility experiments in real-world moving scenarios. We provide potential defense measures that can be implemented at both the sensor level and the vehicle system level to mitigate the risks associated with IEMI attacks. Video demonstrations can be viewed at https://sites.google.com/view/phantomlidar.

==> sections/AttackSummary.tex <==
% !TEX root = ../EM-LiDAR.tex

\subsection{Summary of Attack}
Overall, we can achieve four types of attack effcts:  \textit{Points Interference, Points Removal, LiDAR Power-Off}, and \textit{Points Injection}. 

==> sections/countermeasures.tex <==
% !TEX root = ../EM-LiDAR.tex

\section{Countermeasures}

==> sections/relatedwork.tex <==
% !TEX root = ../EM-LiDAR.tex

\section{Related Work}

\subsection{LiDAR Security}

The output of LiDAR (i.e. point cloud) can be manipulated by laser and 3D object. 
Based on the inherent vulnerability of photoelectric sensors, saturation attack against LiDAR can be easily induced by high-power continuous laser~\cite{shin2017illusion}. After the iterative efforts of several papers~\cite{petit2015remote,shin2017illusion,cao2019adversarial,sun2020towards}, the latest literature~\cite{jin2022pla} proves that a large number of controllable points can be injected into the mechanical (spinning) LiDAR through carefully designed laser pulses, and physically validates the feasibility of hiding attack and creating attack.  However, since lasers share the same physical channel as LiDAR, the ability of lasers to compromise LiDAR systems is an unavoidable phenomenon. This makes it challenging to propose improvements to the safety design of LiDAR systems that would fundamentally prevent laser attacks. Additionally, since laser attacks generally face aiming concerns, the real-world threats of laser attacks has not been widely recognized.
 The way of using 3D objects to manipulate point clouds is also very popular. There are mainly two methods: 3D printing objects and placing arbitrary objects. 3D printing object can realize the adversarial point cloud of specific shape in the physical world, and make the attack difficult to be aware by human beings while spoofing the victim detection model~\cite{cao2019adversarialobject,tu2020physically,yang2021robust}. Some studies have found that for the adversarial attack that aims to hide a target, the position of the adversarial points is more critical than the shape, thus the adversarial effect can be realized by placing the arbitrary object at the specified position~\cite{zhu2021can,zhu2021adversarial}. A recent work~\cite{bhupathiraju2023emi}  demonstrates that EMI can compromise LiDAR’s ToF circuits and induce attack effecrs of "sensor data perturbations". Compared to this work, 
 \alias demonstrates 3 new attack effects with new attack surfaces and signal design methods.
 
 % surfaces including monitoring sensors and optical encoder in beam-steering module

\subsection{IEMI Attacks on Cyber-physical Systems}
Intentional electromagnetic interference (IEMI) attacks can induce parasitic current or voltage into the target cyber-physical systems to manipulate their output data or gain unauthorized access~\cite{tu2019trick,liu2023magbackdoor,kune2013ghost,kasmi2015iemi,dai2023inducing,liu2023magbackdoor,esteves2018remote,fokkens2023prediction,maruyama2019tap,wang2022ghosttouch,shan2022invisible,jiang2022wight,gao2023expelliarmus,jiang2024ghosttype,mohammed2022towards,jiang2023glitchhiker,bhupathiraju2023emi,jang2023paralyzing,pahl2021in,pahl2022analysis,selvaraj2018electromagnetic,dayanikli2022physical,dayanikli2021electromagnetic} and have been of vital interest in recent years.
For example, existing works use IEMI attacks to change the output of microphones~\cite{kune2013ghost,kasmi2015iemi,dai2023inducing,liu2023magbackdoor,esteves2018remote,fokkens2023prediction}, touchscreen~\cite{maruyama2019tap,wang2022ghosttouch,shan2022invisible,jiang2022wight,gao2023expelliarmus}, keyboard~\cite{jiang2024ghosttype} and smart lock~\cite{mohammed2022towards} to allow attackers to inject false speech audios and user inputs, often to pretend that a real user is interacting with the smartphones or computer systems.
Besides, IEMI attacks are also frequently used to change how autonomous systems perceive their surrounding environment, e.g., by changing the output of camera~\cite{jiang2023glitchhiker}  and inertial measurement units~\cite{jang2023paralyzing,pahl2021in,pahl2022analysis,dayanikli2022physical} on autonomous vehicles.

% Both our work and that in~\cite{bhupathiraju2023emi} investigate the IEMI effects on LiDAR sensors. In comparison, our work performs a systematic vulnerability analysis for the effects of the IEMI attacks on LiDAR sensors, designs PhantomLiDAR attacks to demonstrate four categories of attacks, and characterizes the limitations of IEMI attacks against LiDAR sensors.



